Data Voids and Warning Banners on Google Search

The content moderation systems used by social media sites are a topic of widespread interest and research, but less is known about the use of similar systems by web search engines. For example, Google Search attempts to help its users navigate three distinct types of data voids--when the available search results are deemed low-quality, low-relevance, or rapidly-changing--by placing one of three corresponding warning banners at the top of the search page. Here we collected 1.4M unique search queries shared on social media to surface Google's warning banners, examine when and why those banners were applied, and train deep learning models to identify data voids beyond Google's classifications. Across three data collection waves (Oct 2023, Mar 2024, Sept 2024), we found that Google returned a warning banner for about 1% of our search queries, with substantial churn in the set of queries that received a banner across waves. The low-quality banners, which warn users that their results "may not have reliable information on this topic," were especially rare, and their presence was associated with low-quality domains in the search results and conspiracy-related keywords in the search query. Low-quality banner presence was also inconsistent over short time spans, even when returning highly similar search results. In August 2024, low-quality banners stopped appearing on the SERPs we collected, but average search result quality remained largely unchanged, suggesting they may have been discontinued by Google. Using our deep learning models to analyze both queries and search results in context, we identify 29 to 58 times more low-quality data voids than there were low-quality banners, and find a similar number after the banners had disappeared. Our findings point to the need for greater transparency on search engines' content moderation practices, especially around important events like elections.

==> tables/logit/odds-banner_quality-crawl-1-no-impute.tex <==
\begin{tabular}{>{\raggedright\arraybackslash}p{8cm}rlrr}
\toprule
\textbf{Variable} & \textbf{Coef.} & \textbf{95\% CI} & \textbf{Z} & \textbf{P} \\
\midrule
SERP - Average Low-Quality Score & 134.701 & (33.268, 545.403) & 6.872 & 0.000 \\
Query - Conspiracy Keywords (Bool) & 56.390 & (24.686, 128.812) & 9.567 & 0.000 \\
Query - Political Keywords (Bool) & 1.866 & (1.046, 3.329) & 2.112 & 0.035 \\
SERP - Unique Domain Count & 0.962 & (0.881, 1.049) & -0.881 & 0.378 \\
SERP - Rank-weighted News Partisanship & 0.903 & (0.428, 1.907) & -0.266 & 0.790 \\
Query - Character Count (Log10) & 0.878 & (0.573, 1.346) & -0.597 & 0.550 \\
SERP - Estimated Total Results (Log10) & 0.858 & (0.815, 0.904) & -5.813 & 0.000 \\
SERP - Average Domain Traffic (Log10) & 0.821 & (0.753, 0.896) & -4.448 & 0.000 \\
SERP - News Domain Count & 0.614 & (0.516, 0.730) & -5.507 & 0.000 \\
Constant & 0.080 & (0.006, 1.120) & -1.876 & 0.061 \\
\bottomrule
\end{tabular}


==> tables/logit/odds-banner_quality-crawl-2-no-impute.tex <==
\begin{tabular}{>{\raggedright\arraybackslash}p{8cm}rlrr}
\toprule
\textbf{Variable} & \textbf{Coef.} & \textbf{95\% CI} & \textbf{Z} & \textbf{P} \\
\midrule
SERP - Average Low-Quality Score & 568.645 & (107.719, 3001.845) & 7.473 & 0.000 \\
Query - Conspiracy Keywords (Bool) & 35.521 & (11.199, 112.670) & 6.062 & 0.000 \\
Query - Character Count (Log10) & 1.103 & (0.652, 1.867) & 0.366 & 0.714 \\
SERP - Unique Domain Count & 0.980 & (0.860, 1.117) & -0.301 & 0.763 \\
SERP - Estimated Total Results (Log10) & 0.859 & (0.800, 0.923) & -4.144 & 0.000 \\
Query - Political Keywords (Bool) & 0.832 & (0.346, 2.002) & -0.410 & 0.682 \\
SERP - Average Domain Traffic (Log10) & 0.766 & (0.688, 0.852) & -4.920 & 0.000 \\
SERP - News Domain Count & 0.651 & (0.528, 0.802) & -4.023 & 0.000 \\
SERP - Rank-weighted News Partisanship & 0.374 & (0.146, 0.960) & -2.045 & 0.041 \\
Constant & 0.041 & (0.002, 1.127) & -1.889 & 0.059 \\
\bottomrule
\end{tabular}


==> tables/logit/odds-banner_topicality-crawl-1-no-impute.tex <==
\begin{tabular}{>{\raggedright\arraybackslash}p{8cm}rlrr}
\toprule
\textbf{Variable} & \textbf{Coef.} & \textbf{95\% CI} & \textbf{Z} & \textbf{P} \\
\midrule
Query - Character Count (Log10) & 4.606 & (4.326, 4.903) & 47.846 & 0.000 \\
Query - Conspiracy Keywords (Bool) & 4.168 & (2.337, 7.431) & 4.838 & 0.000 \\
Query - Political Keywords (Bool) & 1.841 & (1.657, 2.045) & 11.351 & 0.000 \\
SERP - Average Low-Quality Score & 1.565 & (0.986, 2.485) & 1.900 & 0.057 \\
SERP - Unique Domain Count & 1.045 & (1.025, 1.066) & 4.446 & 0.000 \\
SERP - Average Domain Traffic (Log10) & 0.815 & (0.798, 0.831) & -19.527 & 0.000 \\
SERP - Estimated Total Results (Log10) & 0.796 & (0.788, 0.804) & -43.667 & 0.000 \\
SERP - News Domain Count & 0.728 & (0.708, 0.750) & -21.674 & 0.000 \\
SERP - Rank-weighted News Partisanship & 0.560 & (0.465, 0.674) & -6.130 & 0.000 \\
Query - Contains Operator & 0.014 & (0.004, 0.054) & -6.299 & 0.000 \\
Constant & 0.011 & (0.007, 0.020) & -16.236 & 0.000 \\
\bottomrule
\end{tabular}


==> tables/logit/odds-banner_topicality-crawl-2-no-impute.tex <==
\begin{tabular}{>{\raggedright\arraybackslash}p{8cm}rlrr}
\toprule
\textbf{Variable} & \textbf{Coef.} & \textbf{95\% CI} & \textbf{Z} & \textbf{P} \\
\midrule
Query - Conspiracy Keywords (Bool) & 4.160 & (2.901, 5.965) & 7.753 & 0.000 \\
Query - Character Count (Log10) & 3.237 & (3.081, 3.400) & 46.790 & 0.000 \\
Query - Political Keywords (Bool) & 2.651 & (2.477, 2.838) & 28.118 & 0.000 \\
SERP - Rank-weighted News Partisanship & 1.523 & (1.327, 1.747) & 5.992 & 0.000 \\
SERP - Unique Domain Count & 1.185 & (1.165, 1.204) & 20.283 & 0.000 \\
SERP - News Domain Count & 1.071 & (1.059, 1.083) & 11.820 & 0.000 \\
SERP - Average Domain Traffic (Log10) & 0.899 & (0.885, 0.913) & -13.325 & 0.000 \\
SERP - Estimated Total Results (Log10) & 0.888 & (0.880, 0.895) & -28.212 & 0.000 \\
SERP - Average Low-Quality Score & 0.381 & (0.260, 0.558) & -4.955 & 0.000 \\
Query - Contains Operator & 0.071 & (0.036, 0.138) & -7.788 & 0.000 \\
Constant & 0.001 & (0.001, 0.001) & -31.876 & 0.000 \\
\bottomrule
\end{tabular}


==> tables/logit/odds-banner_topicality-crawl-3-no-impute.tex <==
\begin{tabular}{>{\raggedright\arraybackslash}p{8cm}rlrr}
\toprule
\textbf{Variable} & \textbf{Coef.} & \textbf{95\% CI} & \textbf{Z} & \textbf{P} \\
\midrule
Query - Character Count (Log10) & 4.539 & (4.246, 4.852) & 44.381 & 0.000 \\
Query - Conspiracy Keywords (Bool) & 2.300 & (1.247, 4.243) & 2.666 & 0.008 \\
SERP - Average Low-Quality Score & 1.770 & (1.058, 2.961) & 2.176 & 0.030 \\
SERP - Unique Domain Count & 1.461 & (1.420, 1.503) & 25.951 & 0.000 \\
Query - Political Keywords (Bool) & 1.164 & (1.040, 1.302) & 2.634 & 0.008 \\
SERP - Average Domain Traffic (Log10) & 0.843 & (0.824, 0.862) & -14.663 & 0.000 \\
SERP - News Domain Count & 0.786 & (0.762, 0.811) & -15.150 & 0.000 \\
SERP - Estimated Total Results (Log10) & 0.739 & (0.729, 0.748) & -45.517 & 0.000 \\
SERP - Rank-weighted News Partisanship & 0.502 & (0.415, 0.607) & -7.101 & 0.000 \\
Query - Contains Operator & 0.204 & (0.093, 0.444) & -4.003 & 0.000 \\
Constant & 0.001 & (0.000, 0.001) & -24.487 & 0.000 \\
\bottomrule
\end{tabular}

